ACIC: Admission-Controlled Instruction Cache

The front end bottleneck in datacenter workloads has come under increased scrutiny, with the growing code footprint, involvement of numerous libraries and OS services, and the unpredictability in the instruction stream. Our examination of these workloads points to burstiness in accesses to instruction blocks, which has also been observed in data accesses. Such burstiness is largely due to spatial and short-duration temporal localities, that LRU fails to recognize and optimize for, when a single cache caters to both forms of locality. Instead, we incorporate a small i-Filter as in previous works to separate spatial from temporal accesses. However, a simple separation does not suffice, and we additionally need to predict whether the block will continue to have temporal locality, after the burst of spatial locality. This combination of i-Filter and temporal locality predictor constitutes our Admission-Controlled Instruction Cache (ACIC). ACIC outperforms a number of state-of-the-art pollution reduction techniques (replacement algorithms, bypassing mechanisms, victim caches), providing 1.0223 speedup on the average over a baseline LRU based conventional i-cache (bridging over half of the gap between LRU and OPT) across several datacenter workloads.

==> Sections/Background.tex <==
\section{background}
Data center applications have increasingly complex and deep software stacks, leading to millions of instructions executed to serve a user request. Because of this, the instruction footprints of data center applications are several orders of magnitude larger than the instruction cache size in today's processors~\cite{memory-hierachy-for-web-search}. Frequent i-cache misses significantly degrades the performance of such applications since the long latency accesses to lower cache hierarchies cannot be completely hidden by the out-of-order execution mechanism. Mitigating the performance bottleneck due to i-cache misses can considerably improve the performance of data center applications, resulting in cost and energy savings that are worth millions of dollars.

Reducing i-cache misses has been studied by a number of works in the past few decades~\cite{DBMS-where-does-time-go, reactive-nuca, profile-warehouse, TIFS, PIF, pTask, RDIP}. Prior studies have proposed advanced hardware prefetchers based on temporal prefetching~\cite{TIFS, PIF, Confluence, Boomerang, Shotgun, SHIFT, divide-and-conquer}, software techniques that perform code layout optimizations to improve instruction locality~\cite{Ispike, code-layout-optimization, lightweight-feedback-directed, AutoFDO, optimal-function-placement, BOLT}, and some recent profile-guided prefetching techniques~\cite{AsmDB, I-SPY}. Prefetchers can reduce the long latencies spent in frontend, but very few works have studied the pollution problem in i-cache, except for GHRP~\cite{GHRP} and Ripple ~\cite{Ripple}, which focus on improving i-cache replacement policy by predicting blocks' reuse behavior, and identifying program contexts that are likely to lead to cache misses, respectively.
